An Empirical Study of Vulnerability Detection using Federated Learning

Although Deep Learning (DL) methods becoming increasingly popular in vulnerability detection, their performance is seriously limited by insufficient training data. This is mainly because few existing software organizations can maintain a complete set of high-quality samples for DL-based vulnerability detection. Due to the concerns about privacy leakage, most of them are reluctant to share data, resulting in the data silo problem. Since enables collaboratively model training without data sharing, Federated Learning (FL) has been investigated as a promising means of addressing the data silo problem in DL-based vulnerability detection. However, since existing FL-based vulnerability detection methods focus on specific applications, it is still far unclear i) how well FL adapts to common vulnerability detection tasks and ii) how to design a high-performance FL solution for a specific vulnerability detection task. To answer these two questions, this paper first proposes VulFL, an effective evaluation framework for FL-based vulnerability detection. Then, based on VulFL, this paper conducts a comprehensive study to reveal the underlying capabilities of FL in dealing with different types of CWEs, especially when facing various data heterogeneity scenarios. Our experimental results show that, compared to independent training, FL can significantly improve the detection performance of common AI models on all investigated CWEs, though the performance of FL-based vulnerability detection is limited by heterogeneous data. To highlight the performance differences between different FL solutions for vulnerability detection, we extensively investigate the impacts of different configuration strategies for each framework component of VulFL. Our study sheds light on the potential of FL in vulnerability detection, which can be used to guide the design of FL-based solutions for vulnerability detection.

==> motivation.tex <==
% \section{Motivation}
% \label{motivation}
% The utilization of data-driven, DL-based vulnerability detection methods is often hindered by the inadequate quality and quantity of vulnerability data used for training in practical scenarios~\cite{vdbfl}, thus impacting the model's detection capability. This is due to the issue of data silos formed by users in the domain being unwilling to disclose their privacy-related data. Consequently, the necessity arises to introduce federated learning to encourage users to participate in global model training without sharing their private data.

% The existing federated vulnerability detection method~\cite{vdbfl} is designed for GNNs and their related improved models. However, LLMs' capabilities have progressed in various fields, including vulnerability detection, with their rapid development in recent years. Many Works such as~\cite{vuldebert, vulgpt, transformervul} demonstrate that utilizing LLMs for detecting codes based on textual forms is a highly promising direction, with the performance of these models surpassing traditional models or GNNs in detection. Furthermore, there is a gradual increase in the local model parameters under FL, and research combining FL with LLMs is also growing. 

% The existing works will encounter three issues when facing new trends. Firstly, there is a lack of a federated LLM vulnerability detection framework based on text-form code, and it remains unclear how much performance improvement it can offer compared to local training. Secondly, the relevant studies have not analyzed the challenges that vulnerability detection tasks may face when deployed into FL, especially the non-IID problem. Thirdly, various factors such as federated algorithms, fine-tuning modes, and types of large models collectively affect the performance of federated frameworks. Yet, previous works have not identified which choices among them are superior. Therefore, we propose VulFed to address the aforementioned three issues, effectively filling the gap in this field. We formulate three specific research questions to correspond to the above issues and conduct analysis and research based on these RQs. The RQs we propose are as follows:


% \textbf{RQ1 (The comprehensive effectiveness of VulFed):} Can the global model provided by VulFed be more effective than single-client training? How does the model's performance difference correlate with the types of vulnerabilities, training data volume, and code semantic complexity?

% \textbf{RQ2 (VulFed's performance facing FL issues):} As a framework for code-related tasks, how will VulFed affected by FL typical issues--the non-IID problems?

% \textbf{RQ3 (Searching for advantageous usage strategies):} How to select the various methods within the framework? How do people find the optimal strategy when targeting different vulnerability detection tasks using VulFed?

==> rebuttal.tex <==
It should be noted that in this work, we expect to achieve evaluation models for vulnerability detection but not security detection. Therefore, the emphasis on training data quality assurance should focus on the portion of vulnerable data. Unlike Devign, Diversevul does not have balanced positive and negative samples, which includes 330k non-vulnerable samples and fewer than 19k vulnerable samples. We selected nearly all vulnerable data except for those belonging to rarely occurring CWE types. As for non-vulnerable data, due to its large quantity, it represents redundant data that does not significantly contribute to improving vulnerability detection capabilities. To better balance our training data, we proportionally selected a small subset of secure samples from the top ten projects ranked by commit count, as mentioned in the paper. This approach does not significantly impact the model's vulnerability detection capability.


Actually, we have computed the macro-accuracy of the FL model and its improvement relative to a single model (data listed here), which reveals the effectiveness of FL system. On the other hand, while FL does lead to some increase in false positives for secure samples, it is crucial to emphasize that in practical software scenarios, vulnerabilities are generally few in number but have a great impact. During actual vulnerability detection processes, the cost of false positive mitigation is lower compared to the expense of discovering new vulnerabilities. Therefore, the benefits gained from FL far outweigh any adverse effects it may generate.

In RQ1, our evaluation actually encompasses all combinations of LLM and federated algorithms used in the articles. However, their conclusions are similar, and due to space constraints, we only included representative results in the paper. We have provided a more comprehensive display of the experimental results for RQ1 on our project's website. Please visit (website URL) for further details.

In RQ2, compared to the iid scenario, the evaluation of models in non-iid settings shows a decrease in accuracy for most CWE types, with a few experiencing an increase. This situation correlates with the typical complexity of vulnerability types, as illustrated in the statistical tables and examples we provided. For more details, please refer to (URL)

In RQ3, when evaluating LLM, we used source code datasets constructed from FFMPEG/QEMU data sources, code gadget datasets constructed from SARD/NVRD data sources, and the SEVC dataset, as mentioned in the first row of tables 7 and 8. For GNN model evaluation, inputs were uniformly constructed using the FFMPEG/QEMU data source, as detailed in Section 4.2. Additionally, RQ3 aimed to explore optimal configurations under FL systems, encompassing all related combination experiments in the results section. Differentiated pairing strategies between LLM and PEFT are unrelated to FL and, therefore, do not require evaluation in this context.

In the field of FL, the number of clients does have a significant impact on model performance. Our study actually includes evaluation results across different numbers of clients. However, we believe that the research on how the number of clients affects FL systems has been sufficiently comprehensive, and additional adjustments to this variable in our evaluations would not provide further insights to our study, so we did not include the related data in the article. In response to this issue, we provide the related data at (URL), and we will consider incorporating it into the paper if deemed necessary in subsequent revisions.

The insights gained from our study are not merely specific conclusions dependent on data or methods. Our proposed VulFed framework constitutes a significant contribution to vulnerability detection in FL systems. Moreover, this framework offers high scalability, facilitating the seamless integration of new methods and models to synchronize with updates effectively.

Currently, our study evaluates the model based on the form of binary classification tasks. However, we must emphasize that the core contribution of this paper lies in introducing the first comprehensive framework that integrates FL with vulnerability detection and explores the properties resulting from combining these two domains. We have invested a substantial amount of effort, time, and resources into this endeavor. Expanding the task objectives to fine-grained classification is a goal for our future work. We aim to advance in subsequent efforts rather than encompassing all aspects within the same study.


The conclusions drawn from this study are generalizable. Within the framework VulFed we proposed, we diversified our selection of data sources, datasets, and preprocessing methods as much as possible. Concerning models, we opted for typical lightweight versions of three transformer architectures: encoder-only, decoder-only, and encoder-decoder. For training strategies, we employed various PEFT methods compatible with LLMs. In terms of algorithms, we chose multiple FL algorithms based on different principles, including some of the latest innovations. Therefore, significant effort has been devoted to our research domain to achieve generalizable conclusions. As methods and models continue to evolve in the future, our conclusions are expected to change accordingly. However, as of now, they retain their relevance as a point of reference.

According to RQ1 and the additional results available at (URL), the answer is affirmative. Using FL, compared to a single model, enhances the performance of detecting samples belonging to any CWE type within Diversevul that has a sufficient number of training samples. Additionally, the overall performance across all test data also shows significant improvement. The only negative impact observed is a slight increase in false positive rates for benign samples, which is not deemed unacceptable, as discussed in answer to Weakness 2.

It must be emphasized that in this study, we utilized six different lightweight LLMs, not just CodeBERT. In RQ1 and RQ2, due to similar conclusions across different models and limitations in article length, we focused our analysis on representative models. In RQ3, we combined all types of LLMs we selected with FL algorithms to explore more optimal configurations. Therefore, the conclusions drawn from our study are robust and credible.

Indeed, in the FL domain, there are instances where different participants use models with varying architectures or training levels, which is known as the model heterogeneity problem. However, the issue of model heterogeneity is also recognized as highly complex within the traditional FL domain. Our study currently focuses on approaches with homogeneous models, but we plan to address heterogeneous aspects in future work.

The combination of FL with vulnerability detection in real-world scenarios indeed holds significant potential demand. As you mentioned, data in this field is admittedly limited at present, but with the increasing development of software and code, both generic and specialized data volumes are expected to grow. On the other hand, leveraging pre-trained LLMs allows an efficient adaption to domains with minimal training samples, reducing the risk of overfitting. Therefore, the concerns raised do not undermine the contribution of our research in terms of its generalizability.

We must note that, at the stage when this study reached its main part, CodeLlama had not yet been proposed. Additionally, the large scale of the latest models introduced in recent years poses significant costs in resource-intensive FL systems, making it impractical for us to integrate these models into our framework in the short term. However, we plan to further refine the framework and deploy these models in the final version.
